Trapped by Their Own Rollouts: Understanding Aggregation--Rollout Feedback in Federated On-Policy Distillation

On-policy distillation (OPD) is a promising approach to language-model adaptation, aligning teacher supervision with the student's own generated trajectories. When adaptation prompts are distributed across clients, can this process benefit from federated collaboration? We study federated OPD and find that substantial collaboration gains can be obscured by learning-rate sensitivity: FedAvg can perform no better than independent local training at a small learning rate, yet recover a clear advantage at a larger rate. We explain this phenomenon through the student's dual role as learner and generator of future training data. An aggregation-induced optimization lag can delay access to useful teacher supervision, which in turn slows subsequent learning. Our theory establishes this aggregation--rollout feedback in a solvable model with a common optimum and stable updates, and identifies two coupled roles of learning rate: learning from current supervision and reaching future supervision. Guided by this analysis, we propose FedTOPS (Federated Teacher-guided On-Policy Scaling), which reuses teacher feedback on current trajectories to adapt the FedAvg update magnitude under clientwise predictive-change constraints. Across six mathematical reasoning benchmarks, FedTOPS improves macro Avg@8 over FedAvg by 4.56--14.57 percentage points across the evaluated student models and local learning rates.

==> tables/fixed_benchmarks.tex <==
\begin{table}[htbp]
\centering\small
\caption{Per-benchmark accuracy of fixed-scale controls: Avg@8 / Pass@8 (\%). Macro weights all six benchmarks equally.}
\label{tab:fixed_benchmarks}
\setlength{\tabcolsep}{7pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lcccc}
\toprule

\rowcolor{headbg}\textbf{Benchmark} & \textbf{1$\times$LR, $a=3$} & \textbf{1$\times$LR, $a=10$} & \textbf{3$\times$LR, $a=3$} & \textbf{3$\times$LR, $a=10$}\\
\midrule
MATH500 & 31.80 / 69.00 & 44.12 / 71.40 & 45.20 / 73.00 & 32.40 / 69.80\\
AMC23 & 14.37 / 42.50 & 21.25 / 52.50 & 20.00 / 55.00 & 14.69 / 42.50\\
Minerva & 8.04 / 28.31 & 12.87 / 30.15 & 14.38 / 31.99 & 8.73 / 29.04\\
OlympiadBench & 9.40 / 31.90 & 15.56 / 35.91 & 15.49 / 35.76 & 10.00 / 32.49\\
AIME24 & 0.42 / 3.33 & 2.08 / 13.33 & 1.67 / 6.67 & 0.83 / 3.33\\
AIME25 & 0.83 / 6.67 & 1.25 / 6.67 & 1.67 / 13.33 & 1.25 / 6.67\\
\midrule
Six-benchmark Macro & 10.81 / 30.28 & 16.19 / 34.99 & 16.40 / 35.96 & 11.32 / 30.64\\
\bottomrule\end{tabular}
\end{adjustbox}\end{table}


==> tables/fixed_caps.tex <==
\begin{table}[htbp]
\centering\small
\caption{Cap-hit rates of fixed-scale controls (\%, lower is better) under the common 8,192-token evaluation limit. Red dashes mark unavailable cap-hit statistics.}
\label{tab:fixed_caps}
\setlength{\tabcolsep}{7pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lcccc}
\toprule

\rowcolor{headbg}\textbf{Benchmark} & \textbf{1$\times$LR, $a=3$} & \textbf{1$\times$LR, $a=10$} & \textbf{3$\times$LR, $a=3$} & \textbf{3$\times$LR, $a=10$}\\
\midrule
MATH500 & 29.23 & 27.65 & 18.35 & \pending\\
AMC23 & 28.44 & 41.88 & 32.81 & \pending\\
Minerva & 41.27 & 19.39 & 10.43 & \pending\\
OlympiadBench & 37.00 & \pending & 38.84 & \pending\\
AIME24 & 41.25 & 67.92 & 60.00 & \pending\\
AIME25 & 44.58 & 67.50 & 64.58 & \pending\\
\bottomrule\end{tabular}
\end{adjustbox}\end{table}


==> tables/fixed_controls.tex <==
\begin{table}[htbp]
\centering\small
\caption{\textbf{Fixed-scale controls with the 0.6B student.} Scores are percentages. Best and second-best available values within each learning rate are bold and underlined. Cap hit is lower-is-better. Red dashes mark unavailable cap-hit statistics.}
\label{tab:fixed_controls}
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llrrrrr}
\toprule

\rowcolor{headbg} &  & \multicolumn{3}{c}{\textbf{\textbf{MATH500}}} & \multicolumn{2}{c}{\textbf{\textbf{Six-benchmark Macro}}}\\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}
\rowcolor{headbg}\textbf{Local LR} & \textbf{Method} & \textbf{Avg@8 $\uparrow$} & \textbf{Pass@8 $\uparrow$} & \textbf{Cap hit $\downarrow$} & \textbf{Avg@8 $\uparrow$} & \textbf{Pass@8 $\uparrow$}\\
\midrule
1$\times$ & FedAvg & 11.75 & 51.80 & 54.27 & 3.91 & 19.17\\
1$\times$ & Fixed $a=3$ & 31.80 & 69.00 & 29.23 & 10.81 & 30.28\\
1$\times$ & Fixed $a=10$ & \underline{44.12} & \underline{71.40} & \underline{27.65} & \underline{16.19} & \textbf{34.99}\\
\rowcolor{oursbg}1$\times$ & \textbf{FedTOPS} & \textbf{45.98} & \textbf{72.40} & \textbf{18.75} & \textbf{16.84} & \underline{34.69}\\
\midrule
3$\times$ & FedAvg & 37.28 & 72.00 & 21.93 & 12.78 & 31.62\\
3$\times$ & Fixed $a=3$ & \underline{45.20} & \textbf{73.00} & \underline{18.35} & \underline{16.40} & \textbf{35.96}\\
3$\times$ & Fixed $a=10$ & 32.40 & 69.80 & \pending & 11.32 & 30.64\\
\rowcolor{oursbg}3$\times$ & \textbf{FedTOPS} & \textbf{47.02} & \underline{72.20} & \textbf{13.68} & \textbf{17.33} & \underline{35.50}\\
\bottomrule\end{tabular}\end{adjustbox}\end{table}


==> tables/main_06b_lr1_avg_at_8_rows.tex <==
Local C1 & \textbf{12.93} & \underline{4.06} & \underline{3.58} & \textbf{4.58} & \textbf{0.83} & \textbf{0.42} & \textbf{4.40}\\
Local C2 & 11.47 & \textbf{4.69} & \textbf{3.68} & 4.08 & \underline{0.42} & 0.00 & 4.06\\
Local C3 & \underline{12.65} & 3.12 & 3.45 & 4.30 & 0.00 & 0.00 & 3.92\\
Local mean & 12.35 & 3.96 & 3.57 & \underline{4.32} & \underline{0.42} & \underline{0.14} & \underline{4.13}\\


==> tables/main_06b_lr1_max_length_hit_rate_rows.tex <==
Base student & 50.68 & 46.88 & 48.85 & 51.91 & \underline{52.08} & 51.25 & 50.27\\
\midrule
Centralized & \underline{30.12} & \underline{35.31} & \underline{41.13} & \textbf{37.11} & \textbf{42.50} & \textbf{42.92} & \textbf{38.18}\\
Local C1 & 53.12 & 57.19 & 50.69 & 53.36 & 55.00 & \underline{49.17} & 53.09\\
Local C2 & 55.85 & 55.31 & 52.53 & 56.31 & 59.17 & 53.75 & 55.49\\
Local C3 & 54.43 & 57.81 & 51.98 & 54.75 & 55.83 & 56.25 & 55.17\\
Local mean & 54.47 & 56.77 & 51.73 & 54.80 & 56.67 & 53.06 & 54.58\\
FedAvg & 54.27 & 55.62 & 51.79 & 54.27 & 58.33 & 55.00 & 54.88\\
\rowcolor{oursbg}\textbf{FedTOPS} & \textbf{18.75} & \textbf{30.31} & \textbf{10.48} & \underline{38.22} & 69.17 & 62.92 & \underline{38.31}\\


==> tables/main_06b_lr1_pass_at_8_rows.tex <==
Local C1 & \underline{52.40} & \textbf{27.50} & \underline{18.38} & \textbf{23.00} & \textbf{3.33} & \textbf{3.33} & \textbf{21.32}\\
Local C2 & 50.40 & \underline{25.00} & \textbf{19.49} & 22.11 & \textbf{3.33} & 0.00 & \underline{20.05}\\
Local C3 & \textbf{53.00} & 15.00 & 16.54 & \underline{22.55} & 0.00 & 0.00 & 17.85\\
Local mean & 51.93 & 22.50 & 18.14 & \underline{22.55} & \underline{2.22} & \underline{1.11} & 19.74\\


==> tables/main_06b_lr3_avg_at_8_rows.tex <==
Local C1 & \textbf{33.70} & \textbf{16.56} & \textbf{8.32} & \textbf{10.65} & 0.83 & 0.42 & \textbf{11.75}\\
Local C2 & 22.15 & 10.94 & 6.16 & 6.36 & 0.83 & \textbf{1.67} & 8.02\\
Local C3 & 24.45 & 11.88 & 6.76 & 7.10 & \textbf{1.67} & 0.00 & 8.64\\
Local mean & \underline{26.77} & \underline{13.12} & \underline{7.08} & \underline{8.04} & \underline{1.11} & \underline{0.69} & \underline{9.47}\\


==> tables/main_06b_lr3_max_length_hit_rate_rows.tex <==
Base student & 50.68 & 46.88 & 48.85 & 51.91 & 52.08 & 51.25 & 50.27\\
\midrule
Centralized & 29.62 & 46.88 & \underline{20.08} & 51.41 & 70.00 & 73.75 & 48.62\\
Local C1 & 25.00 & 29.06 & 35.80 & 33.10 & \underline{40.83} & \underline{38.33} & 33.69\\
Local C2 & 44.85 & 50.94 & 50.14 & 51.19 & 53.75 & 56.25 & 51.19\\
Local C3 & 40.88 & 43.44 & 48.39 & 49.59 & 53.33 & 51.25 & 47.81\\
Local mean & 36.91 & 41.15 & 44.78 & 44.63 & 49.31 & 48.61 & 44.23\\
FedAvg & \underline{21.93} & \textbf{26.25} & 32.26 & \underline{29.88} & \textbf{40.42} & \textbf{36.25} & \textbf{31.16}\\
\rowcolor{oursbg}\textbf{FedTOPS} & \textbf{13.68} & \underline{28.44} & \textbf{7.90} & \textbf{29.47} & 53.75 & 54.17 & \underline{31.23}\\


==> tables/main_06b_lr3_pass_at_8_rows.tex <==
Local C1 & \textbf{69.20} & \textbf{47.50} & \textbf{26.47} & \textbf{35.01} & 6.67 & 3.33 & \textbf{31.36}\\
Local C2 & 64.80 & 42.50 & 23.16 & 27.60 & 6.67 & \textbf{10.00} & 29.12\\
Local C3 & \underline{67.00} & \underline{45.00} & \underline{25.00} & 28.64 & \textbf{10.00} & 0.00 & 29.27\\
Local mean & \underline{67.00} & \underline{45.00} & 24.88 & \underline{30.42} & \underline{7.78} & \underline{4.44} & \underline{29.92}\\


==> tables/scaleup_17b_avg_at_8_rows.tex <==
Local C1 & \underline{29.43} & 15.31 & 9.65 & \textbf{12.31} & 2.50 & 1.25 & 11.74\\
Local C2 & \textbf{30.03} & \textbf{17.19} & \textbf{10.62} & \underline{12.18} & \textbf{3.33} & 0.83 & \textbf{12.36}\\
Local C3 & 28.78 & 14.37 & 10.02 & 11.48 & \underline{2.92} & \textbf{2.08} & 11.61\\
Local mean & 29.41 & \underline{15.62} & \underline{10.09} & 11.99 & \underline{2.92} & \underline{1.39} & \underline{11.90}\\


==> tables/scaleup_17b_max_length_hit_rate_rows.tex <==
Centralized & \textbf{4.17} & \textbf{6.25} & \underline{2.90} & \textbf{8.46} & \underline{20.42} & \textbf{11.67} & \textbf{8.98}\\
Local C1 & \underline{37.05} & 38.75 & 32.72 & 39.52 & 40.42 & 42.08 & 38.42\\
Local C2 & 37.77 & 39.69 & 32.31 & 39.47 & 39.58 & 43.75 & 38.76\\
Local C3 & 37.50 & 40.31 & 32.86 & 40.49 & 44.17 & 42.50 & 39.64\\
Local mean & 37.44 & 39.58 & 32.63 & 39.82 & 41.39 & 42.78 & 38.94\\
FedAvg & 38.15 & 38.44 & 33.13 & 40.13 & 40.42 & 41.67 & 38.66\\
\rowcolor{oursbg}\textbf{FedTOPS} & \textbf{4.17} & \underline{9.06} & \textbf{2.57} & \underline{8.55} & \textbf{19.17} & \underline{15.83} & \underline{9.89}\\


==> tables/scaleup_17b_pass_at_8_rows.tex <==
Local C1 & 74.60 & 55.00 & 33.82 & \textbf{40.80} & \textbf{16.67} & \underline{10.00} & \underline{38.48}\\
Local C2 & \textbf{76.40} & \textbf{65.00} & \underline{35.66} & 40.06 & 13.33 & 6.67 & \textbf{39.52}\\
Local C3 & 74.60 & 47.50 & \textbf{36.03} & 39.91 & 13.33 & \textbf{13.33} & 37.45\\
Local mean & \underline{75.20} & \underline{55.83} & 35.17 & \underline{40.26} & \underline{14.44} & \underline{10.00} & \underline{38.48}\\

